Accelerating Generalized Linear Models with MLWeaving: A One-Size-Fits-All System for Any-precision Learning (Technical Report)

Learning from the data stored in a database is an important function increasingly available in relational engines. Methods using lower precision input data are of special interest given their overall higher efficiency but, in databases, these methods have a hidden cost: the quantization of the real value into a smaller number is an expensive step. To address the issue, in this paper we present MLWeaving, a data structure and hardware acceleration technique intended to speed up learning of generalized linear models in databases. ML-Weaving provides a compact, in-memory representation enabling the retrieval of data at any level of precision. MLWeaving also takes advantage of the increasing availability of FPGA-based accelerators to provide a highly efficient implementation of stochastic gradient descent. The solution adopted in MLWeaving is more efficient than existing designs in terms of space (since it can process any resolution on the same design) and resources (via the use of bit-serial multipliers). MLWeaving also enables the runtime tuning of precision, instead of a fixed precision level during the training. We illustrate this using a simple, dynamic precision schedule. Experimental results show MLWeaving achieves up to16 performance improvement over low-precision CPU implementations of first-order methods.

==> bit_serial.tex <==
\section{Bit-Serial Method (BSM)} %: Flexibility \& Performance
\label{sec_bit_serial_method}
%In this section, we try to achieve the objective that the overall performance scales linearly with the number of bits used. Then, the fundamental question we want to answer in this section is how to technically achieve the linear scalability with only one hardware design, while incurring trivial storage and hardware overhead. 
%%we present the key technique (i.e., bit-serial method), which enables
In this section, we present BSM, which achieves the objective that both memory access and computation time scales linearly with the number of bits used for low-precision ML. BSM contains its own memory layout and arithmetic. % 
\vspace{-1ex}
\subsection{BSM Memory Layout (Software)}% (Software Component)
%{\bf Objective. }
%Inspired by BitWeaving, 
The BSM memory layout is based on ideas proposed by BitWeaving~\cite{bitweaving_sigmod13, widetable_vldb14}. In a nutshell, we transpose the training dataset to allow the run time selection of the level of precision and to reduce memory traffic for lower precision levels. 
Contrary to BitWeaving, which performs the weaving on one column, BSM transposes each row (a sample) to preserve access locality, since the training dataset is accessed by SGD in a \emph{sample-at-a-time} manner. %the bit-level columnar organization
%Based on the execution pattern of SGD in Algorithm~\ref{alg_sgd_flow}, 
%accesses data in a column-major
%The format aims at requiring only one indexing operation to support any level of precision (bit-level flexibility). Second, the memory access time decreases linearly as less bits are used. We present the bit-serial storage layout, followed by the related memory access pattern. 


%In order to preserve the access locality, we perform the weaving on the sample to achieve the bit-level flexibility. 
The transposition of the data used in BSM is shown in Figure~\ref{fig_bit_serial_layout}. $M$ $S$-bit features of a sample are transposed into $S$ $M$-bit words (where $M$ is 8 and $S$ is 4 in the example shown).
Inside the first row, eight 4-bit features are transposed into four 8-bit words. The first bits (i.e., {\color{blue} AEIMRV10}) of the first sample are stored in a 8-bit word.
The second word {\color{red} BFJNSX01}, which contains the second bits, is stored next to the first word, and so on.  
Between rows, the second row is stored consecutively to the first row. 

Under the BSM memory layout, data at any level of precision can be retrieved by following a different access pattern over the same data structure. 
%Suppose we train a machine learning algorithm with the $s$-bit precision ($s \le S$), we only need to access $s$ bits for each sample. Figure~\ref{fig_bit_serial_layout} also shows the case that $s$ is equal to 3. 
In Figure~\ref{fig_bit_serial_layout}(b), we show the accesses needed to retrieve the data set at a precision of 3 bits. The first bits in the first row are accessed, followed by the second and third bits. Then, the access jumps to the first bits of the second row, skipping the fourth bits of each row. %Acquiring all the bytes for one value in a given dimension or feature (a column entry) involves sequential memory access, which improves overall performance.  %Therefore, three words are referenced for each sample. 

%In summary, we observe that our objective is accomplished. \emph{The proposed bit-serial storage layout (i.e., one index) can support the flexible selection of precision. The memory access time decreases linearly as a lower number ($s$) of bits is used}.    
%This is {\color{blue} highlighted}, and this is not. flexibility of

%\kaancomment{Should we talk about this padding overhead and whether it is absolutely necessary?: In the current setting, the padding creates a large memory usage overhead if the number of features are low. However, this can be improved by decreasing the line granularity we are operating from 64 Bytes to 32 Bytes or lower, with minor modifications to our design.}[-3cm]
{\bf Instantiation of Memory Layout. } Table~\ref{t_bit_serial_instance} shows an example of a BSM memory layout with $\#CL$ = 512 and $M$ (number of features) = 2048. For instance, the first memory slot (with index = 0) is populated with the first bits of the first 512 features of the first sample, while the second memory slot (with index = 1) is populated with he second bits of the first 512 features of the first sample.  If $M$ is not a multiple of 512, we use padding to fit a 512-bit boundary. %\emph{x\_y:z\_w} denotes the \emph{w}-th bits of 512 features (from $z$-th to $y$-th) in the $x$-th sample and $y - z = 511$.  

\begin{figure}[t]
	\centering
	\includegraphics[width=8cm]{bit_serial_storage_lyout_memory_access_pattern.pdf}
	\vspace{-2.0ex} %bit_serial_layout
	\caption{Full-precision fixed-point memory layout (a) converted into the BSM memory layout (b). Each symbol (e.g., A-Z, a-z) in the table is binary, 0 or 1. The BSM memory layout enables the flexible selection of precision in memory. As an example, we show the ``memory access pattern'' with a 3-bit precision ($s$ = 3). }
	\vspace{-4ex} 
	\label{fig_bit_serial_layout}
\end{figure}

\begin{table} %[!h]
	\centering
	%\begin{spacing}{0.3}
	\begin{scriptsize}
		\begin{tabular}{|p{2cm}|c||c|}
			\hline
			\textbf{Description} &\textbf{Index} & \textbf{Content ($\#CL$=512 bits)} \\%
			\hline
			\hline
			\hline
			\multirow{6}={First 512 features of the first sample} & $0$ & 0\_511:0\_0\\
			\cline{2-3}
			& $1$ & 0\_511:0\_1\\
			\cline{2-3}
			& $2$ & 0\_511:0\_2\\
			\cline{2-3}
			&$3$ & 0\_511:0\_3\\
			\cline{2-3}
			& $...$ & ... \\
			\cline{2-3}
			& $31$ & 0\_511:0\_31\\
			\hline
			\hline
			\multirow{4}={Second 512 features of the first sample} & $32$ & 0\_1023:512\_0\\
			\cline{2-3}
			&$33$ & 0\_1023:512\_1\\
			\cline{2-3}
			&$34$ & 0\_1023:512\_2\\
			\cline{2-3}
			&$...$ & ... \\
			\hline
			\hline
			$...$&$...$ & ... \\
			\hline
			\hline			\multirow{3}={First 512 features of the second sample} & $128$ & 1\_511:0\_0\\
			\cline{2-3}
			&$129$ & 1\_511:0\_1\\
			\cline{2-3}
			& $...$ & ... \\
			\hline
		\end{tabular}
	\end{scriptsize}
	\vspace{-1ex}
	\caption{Instantiation of BSM memory layout. \emph{x\_y:z\_w} denotes the \emph{w}-th bits of 512 features (from $z$-th to $y$-th) in the $x$-th sample.}% and $y - z = 511$
		\vspace{-2ex}
		\label{t_bit_serial_instance}
\end{table}

% \begin{table} %[!h]
% 	\centering
% 	%\begin{spacing}{0.3}
% 	\begin{scriptsize}
% 		\begin{tabular}{|c||c|c|}
% 			\hline
% 			\textbf{Index} & \textbf{Content ($\#CL$=512 bits)} \\%
% 			\hline
% 			\hline
% 			\hline
% 			$0$ & 0\_511:0\_0\\
% 			\hline
% 			$1$ & 0\_511:0\_1\\
% 			\hline
% 			$2$ & 0\_511:0\_2\\
% 			\hline
% 			$3$ & 0\_511:0\_3\\
% 			\hline
% 			$...$ & ... \\
% 			\hline
% 			$31$ & 0\_511:0\_31\\
% 			\hline
% 			\hline
% 			$32$ & 0\_1023:512\_0\\
% 			\hline
% 			$33$ & 0\_1023:512\_1\\
% 			\hline
% 			$34$ & 0\_1023:512\_2\\
% 			\hline
% 			$...$ & ... \\
% 			\hline
% 			\hline
% 			$128$ & 1\_511:0\_0\\
% 			\hline
% 			$129$ & 1\_511:0\_1\\
% 			\hline
% 			$...$ & ... \\
% 			\hline
% 		\end{tabular}
% 	\end{scriptsize}
% 	\vspace{-1ex}
% 	\caption{Instantiation of BSM memory layout. \emph{x\_y:z\_w} denotes the \emph{w}-th bits of 512 features (from $z$-th to $y$-th) in the $x$-th sample and $y - z = 511$.}
% 		\vspace{-3ex}
% 		\label{t_bit_serial_instance}
% 	%\end{spacing}
% \end{table}
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=7.1cm]{bit_serial_memory_access_pttern.pdf}
%	\vspace{-1.5ex}
%	\caption{Memory access pattern under bit-serial method. An example of accessing table with the 3-bit precision ($s$ = 3). }
%	\vspace{-2ex}
%	\label{fig_bit_serial_memory_access}
%\end{figure}

%One thing needs to be mentioned is that the data from the bit-serial storage layout is in a bit serial stream. In other words, the entire feature is not atomically fetched in a cycle. The first bit arrives at the first cycle, the second bit arrives at the second cycle, and so on. 

%Since the memory access    

%However, for the machine learning computing task (training or inference), it needs to reference all the features of a sample to compute the loss. Essentially, full-precision is not necessary for the classification. So it is getting more and more popular to use low-precision data representation for machine learning computing task. 
%
%New Layout:::
%
%Original-->32-bit -> 8-bit.  HBP
%are
%Our     -->                  VBP
%
%During the normalization, we perform the weaving on the training dataset.   
%
%The first bit means the 0.5.
\vspace{-1ex}
\subsection{BSM Arithmetic (Hardware)} % (Hardware Component)
%Therefore, it can achieve the bit-level flexibility, i.e., supporting any level of precision with a single hardware design. %imports the bit-serial multiplier into our hardware design.

Using a bit-serial multiplier operating on the data one bit per cycle~\cite{stripes_micro16, convnets_vlsic16, filter_adaptive_precision_asicsoc99, bismo_fpl18, bit_serial_assp89, dct_vlsi99}, we design the BSM arithmetic which provides bit-level flexibility (i.e., supporting any precision with a single hardware design) while maintaining a processing rate of a cache line per clock cycle. %. %Besides, the computation time of scales linearly as less bits are used. 
%The objective of bit-serial arithmetic is two-fold. First, only one hardware design is used to . Second,
We now present the difference between bit-serial and bit-parallel multipliers, followed by the SGD arithmetic powered by bit-serial multiplier.  

%the computation time scales linearly with the number of bits used. 

{\bf Bit-serial Multiplier vs. Bit-parallel Multiplier}.  
We illustrate the difference between a bit-parallel multiplier and a bit-serial multiplier with one example multiplying $3$-bit $Q_3(a)$ (low-precision) by $4$-bit $x$ (full-precision) (Figure~\ref{fig_bit_serial_vs_paralle}). %Here, 

%Suppose we want to , and w
In a bit-parallel multiplier, each clock cycle can enable the multiplication of two numbers, in this case the quantized input $Q_{3}(a)$ and the corresponding value from the model $x$ (Figure~\ref{fig_bit_serial_vs_paralle}a). This is the type of multiplier used in conventional CPUs and also previous specialized hardware solutions~\cite{sgd_fpga_fccm17}. %However, it cannot efficiently support another level of precision, except $s$-bit.

\wzk{In a bit-serial multiplier, one multiplication result is produced every three cycles, a bit of $Q_{3}(a)$ per cycle. After $Q_3(a)$ is replaced with $\sum_{i=1}^{3} a^{[i]} \times 2^{-i}$ in Equation~\ref{equ_bit_comp}}, the product $Q_3(a) \times x$ in Equation~(\ref{E_bit_serialmultiplication}) is computed to be the sum of the product of $a^{[i]}$ and ($x \ggg i$), where the binary value $a^{[i]}$ represents the $i$-th bit of $a$ (0 or 1), $\ggg$ means the signed right shift, and $i$ is from 1 to 3. 
%The first bit is the most significant bit.  within three cycles
\begin{equation} \begin{scriptsize}
\label{E_bit_serialmultiplication}
	\vspace{-1ex}
Q_3(a) \times x = x \times \sum_{i=1}^{3} a^{[i]} \times 2^{-i} = \sum_{i=1}^{3} a^{[i]} \times (x \ggg i)
	\vspace{-2ex}
\end{scriptsize} \end{equation}
In terms of cycles, the product $Q_3(a) \times x$ is set to be $a^{[1]} \times (x \ggg 1)$ on the first cycle, $a^{[2]} \times (x \ggg 2)$ is added to the product on the second cycle, and $a^{[3]} \times (x \ggg 3)$ is added on the third cycle. The advantage of bit-serial multiplier is that shift-and-add operations are enough for the calculation, considerably simplifying the design. The disadvantage is that more cycles are needed to complete the operation.

%We can see that $x$ enters the bit-serial multiplier in a bit-parallel fashion, while $Q_3(a)$ enters in a bit-serial fashion in Figure~\ref{fig_bit_serial_vs_paralle}b. %Therefore, its throughput is three cycles per product.
\begin{figure}[t]
	\centering
	\includegraphics[width=9.1cm]{bit_serial_vs_parallel.pdf}
	\vspace{-3.5ex}
	\caption{Multipliers: bit-parallel (a) vs. bit-serial (b). Bit-parallel multiplier produces one multiplication result per cycle, while bit-serial multiplier produces every three cycles, e.g., on cycle 3 or 6. }
	\vspace{-3.5ex}
	\label{fig_bit_serial_vs_paralle}
\end{figure}
%The bit-parallel multiplier can produce one product per cycle, compared with three cycles per product of the bit-serial multiplier.

%Suppose we want to multiply $B$-bit $Q_B(a)$ (low-precision) by $S$-bit $x$ (full-precision), and we identify the difference between bit-parallel multiplier and bit-serial multiplier. %Here, 
%
%{\bf Bit-parallel multiplier. } Originally, the custom fixed-width bit-parallel multiplier ($B \times S$) is employed to do the computation. Its throughput is one product per cycle. However, it cannot efficiently support another level of precision, except $B$-bit.  
%
%{\bf Bit-serial multiplier. }
%Under bit-serial mulitplier, replacing $Q_B(a)$ with the value in Equation~\ref{E_number_representation}, its product ($ax$) is computed to be the sum of $B$ terms, each of which can be calculated using simple shift and And operations, as shown in Equation~\ref{E_bit_serialmultiplication}. 
%\begin{equation} \begin{scriptsize}
%\label{E_bit_serialmultiplication}
%ax = Q_B(a) \times x = x \times \sum_{i=1}^{B} a^{[i]} \times 2^{-i} = \sum_{i=1}^{B} a^{[i]} \times (x \ggg i),
%\end{scriptsize} \end{equation}
%where $\ggg$ means the signed right shift.  
%
%In terms of cycle, the product $ax$ is set to be $a^{[1]} \times (x \ggg 1)$ at the first cycle, $a^{[2]} \times (x \ggg 2)$ is added to $ax$ at the second cycle, and so on. 


{\bf Hardware Design of BSM}. The goal of BSM arithmetic is to accept 512-bit data per cycle from the BSM memory layout described above. According to Algorithm~\ref{alg_sgd_flow}, we implement the fully-pipelined hardware design for the BSM arithmetic, as shown in Figure~\ref{fig_bit_serial_hardware}. In essence, each instruction of SGD occupies unique hardware resources of an FPGA. In the following, we discuss the detailed implementation for each stage. %achieves both flexibility and high performance
%The key idea of the bit-serial arithmetic is to replace bit-parallel multipliers with bit-serial multipliers. (\circled{2}) 
%In the data reading stage, the arithmetic can  This data is fed to the computation pipeline and 

 
%it consumes 512-bit data stream from the BSM memory layout per cycle. In particular,  
In the ``dot product" stage, 512 bit-serial multipliers are instantiated (\circled{1}) to consume the 512-bit data stream (\circled{A}) from the BSM memory layout per cycle, where each bit-serial multiplier can handle a bit from a feature per cycle. At the same time, the data stream is also fed to the ``FIFO" (\circled{B}). On the first cycle, the first bits from the first 512 features from a sample enter the pipeline in a lock-step manner, and 512 values are read from the \emph{architectural model} (labelled $\vec x$ in Figure~\ref{fig_bit_serial_hardware}), where the architectural model stores the committed state of the model $\vec x$ to preserve the semantics of mini-batch SGD. After processing $s$ bits of the first 512 features (where $s$ is the precision level used in the execution), 512 multiplication results are passed to the fully-pipelined adder tree (\circled{2}), whose depth is $log_2(512)$. The output of the adder tree is connected to an accumulator (\circled{3}), which aggregates $\lceil\tfrac{M}{512}\rceil$ valid results from the adder tree and then computes the final result ($Q_s(\vec{a}) \boldsymbol{\cdot} \vec{x}$) of the dot product\footnote{In the actual implementation, we adopt the distributed arithmetic computation approach~\cite{stripes_micro16, bit_serial_assp89} to compute the dot product, since it produces the same result with fewer hardware resources. In the paper, we use the basic bit-serial multiplier for ease understanding. }, where $M$ is number of features in the sample. %, so the degree of intra-sample parallelism is $\#CL$ 

In the ``serial part" stage, the scaling value \emph{scale} (\circled{4}) is computed to be $\lambda \times df(Q_s(\vec{a}) \boldsymbol{\cdot} \vec{x}, b)$, where $\lambda$ is the learning rate (parameterizable at runtime), $df$ is the derivative of the given loss function, and $b$ is the label\footnote{In our actual implementation, we also load the label $b$ from memory. However, we omit the related data path in Figure~\ref{fig_bit_serial_hardware} for clarity.} of the sample.   

In the ``gradient computation" stage, we again instantiate 512 bit-serial multipliers (\circled{5}) to compute the full-precision gradient with comparable throughput to the ``dot product" stage. The scaling value \emph{scale} is broadcast to each bit-serial multiplier as its bit-parallel input, while the bit-serial input $Q_s(\vec{a})$ can be read from the``FIFO" (\circled{B}). The bit-serial multipliers in this stage require exactly the same bit stream order of $Q_s(\vec{a})$ as that in the ``dot product" stage.    

In the ``model update" stage, the part of the gradient from the first 512 features is computed after $s$ cycles, and then used to update the \emph{working model} ($\overrightarrow{x\_w}$). The working model keeps the temporary model updated after each data sample is processed (\circled{6})\footnote{The pair (architectural model, working model) is only used in the hardware design (Figures~\ref{fig_bit_serial_hardware}, \ref{fig_mlweaving_hw}), analogous to the pair (architectural register, physical register) in computer architecture. The architectural register indicates the register specified by instruction set architecture (ISA), visible to the programmer. The physical register is used to store temporary results, invisible to the programmer. }. Later, $\overrightarrow{x\_w}$ is updated with the part of gradient from the second 512 features after next $s$ cycles, and so on. $\overrightarrow{x\_w}$ is updated at the rate of every sample, while the architectural model ($\vec x$) is updated only after a mini batch ($B$) of samples (\circled{7}), where $B$ is the mini batch size (parameterizable at runtime). Therefore, samples in this mini batch are able to read the expected model without any pollution from the gradient of this mini batch; in other words, the semantics of mini-batch SGD is preserved. %It mean that the width of the model 

\begin{figure}[t]
	\centering
	\includegraphics[width=8cm]{bit_serial_hardware.pdf}
	\vspace{-1.5ex}
	\caption{Hardware design of BSM}% For the instantiation, $\#CL$ is 512.
	\vspace{-3ex}
	\label{fig_bit_serial_hardware}
\end{figure}

%{\bf Instantiation of hardware design. }
%We instantiate the bit-serial hardware design by setting $\#CL$ to 512 in Figure~\ref{fig_bit_serial_hardware}.  

%
%\subsubsection{Objective} 
%{\bf Flexibility. }In order to achieve the flexibility we want, we replace bit-parallel fixed-width multipliers with bit-serial multipliers. %(in Figure~\ref{fig_quantizated_hardware})
%
%
%(in the dot product and gradient computation parts in Figure~\ref{fig_bit_serial_hardware})
%
%Since the other components (except the bit-serial multiplier) are kept with the throughput of one result in one cycle, the overall throughput is dominated by the performance of the bit-serial multiplier.
%
%{\bf Performance. }In order to achieve comparable throughput ($\#CL$ bits/cycle), the bit-serial arithmetic has to consume $\#CL$ (e.g., 512) bits  per cycle, each bit for one feature. Therefore, $\#CL$ bit-serial multipliers are instantiated to the dot product to achieve the $\#CL$-way intra-sample parallelism. 
%
%Similarly, the gradient computation part also requires $\#CL$ bit-serial multipliers. Therefore, the achieved processing rate of the bit-serial arithmetic is $\tfrac{\#CL}{s}$ features per cycle, where $s$ is the precision level at runtime.

%Therefore, for one sample with $M$ features, it requires $\lceil\cfrac{M}{\#CL}\rceil * s $ cycles to process, where $s$ is the targeted precision level and $\lceil\cfrac{M}{\#CL}\rceil$ means that the number of features is padded to a $\#CL$-bit boundary. 

%In summary, our objective is accomplished. \emph{The proposed bit-serial arithmetic (i.e., one hardware design) can support the arbitrary-precision training. The computation time scales linearly with the number ($B$) of bits used}.   


%According to Algorithm~\ref{alg_sgd_flow}, the computations of SGD mainly comprise of three vector operations, e.g., $Q_s(\vec{a_i}) \boldsymbol{\cdot} \vec{x}$ (Line 3), $scale \times Q_s(\vec{a_i})$ (Line 5) and $\vec{x} = \vec{x} - \vec{g}$ (Line 6). 
%The main component of vector operation is multiplication.%, whose precision varies in the context of low-precision SGD.     



%Therefore, one product is produced every $B$ cycles. 
%\subsection{Benefits of Hardware/Software Codesign}
%%Therefore, it requires $B$ cycles to compute its product. %The bit-serial compute unit 
%We observe that the bit-serial arithmetic can smoothly consume the bit serial stream (e.g., $a^{[1]}$, $a^{[2]}$, $\dots$, $a^{[B]}$), which is the exact data stream from the proposed bit-serial storage layout (software component). It indicates that no auxiliary hardware resources are required for the ordering, maximizing the energy efficiency. 
%



%One thing to be mentioned is that the throughput with bit-serial arithmetic is much lower than the original bit-parallel arithmetic. In the next section, we prepose \texttt{MLWeaving} to achieve performance while keeping flexibility. 


%Bit-serial enables the flexible selection of precision in hardware, providing $\#CL$-way parallelism. The bitwidth of the model becomes $32 \times \#CL$, causing a serious challenge for the hardware design. 

%Arbitrary-precision arithmetic is considerably slower than bit-parallel arithmetic using numbers that fit entirely within processor registers, since the latter produce one word per cycle whereas the former consumes one bit per cycle. 
%$B$: the number of bits used. we use the bit-serial compute unit, instead of the common bit-parallel multiplier. 

%Essentially, one of the operands is stored in bit-parallel way, 



==> cost_model.tex <==
\section{Cost Model}
In this section, we present a cost model to predict the performance of MLWeaving on FPGAs. We predict the throughput $Th$, which is evaluated to be the minimum value between computing throughput $Th_{comp}$ and memory throughput $TH_{mem}$, as shown in Equation~\ref{E_throughput_overall}.
\begin{equation} \begin{scriptsize}
\label{E_throughput_overall}
\vspace{-1ex}
Th = Min (Th_{comp},Th_{mem})
\vspace{-1ex}
\end{scriptsize} \end{equation}

\subsection{Evaluating Computing Throughput}
In this subsection, we present an analytical model to evaluate the computing throughput for ``with chaining" and ``wo chaining". The MLWeaving hardware design can consume 512 bits per cycles, so its theoretical computing throughput is 512 bits*400MB=25.6GB/s. However, the practical computing throughput is lower, since MLWeaving has to guarantee the RAW dependency regarding the model. One unavoidable factor is the pipeline latency $L$, which is distance between dot product and model updating modules. Its value is $40+2s$ cycles, where $s$ is the precision level. 

%\noindent
{\bf ``With chaining". }We evaluate the computing throughput of ``with chaining", as shown in
Equation~\ref{E_comp_with_chaining}.
\begin{equation} \begin{scriptsize}
\label{E_comp_with_chaining}
\vspace{-1ex}
Th_{comp} = \cfrac{(B/8) \times \lceil M/64\rceil \times s}{(B/8) \times \lceil M/64\rceil \times s + L} \times 25.6GB/s, 
\vspace{-1ex}
\end{scriptsize} \end{equation}
where the right part is the theoretical computing throughput and the left part is the utilization of the computing logic (i.e., dot product module). Since the chaining is enabled, the overhead of model updating can be removed. However, the pipeline latency $L$ cannot be ignored, especially when $M$ and $s$ are small. 

%\noindent
{\bf ``Wo chaining". }Now we evaluate the computing throughput of ``wo chaining", as shown in
Equation~\ref{E_comp_wo_chaining}.
Equation~\ref{E_comp}.
\begin{equation} \begin{scriptsize}
\label{E_comp_wo_chaining}
\vspace{-1ex}
Th_{comp} = \cfrac{(B/8) \times \lceil M/64\rceil \times s}{(1+B/8) \times \lceil M/64\rceil \times s + L} \times 25.6GB/s, 
\vspace{-1ex}
\end{scriptsize} \end{equation}
where the overhead of model updating is $\lceil M/64\rceil \times s$. The dot product is idle when the model updating is active. 

\subsection{Evaluating Memory Throughput}
MLWeaving accesses the host memory via two PCIe and one QPI links, so the memory throughput is impacted by both memory subsystem and PCIe/QPI links. This make the explicit prediction (in terms of analytical cost model) of memory throughput extremely difficult, especially under the condition the memory-related IP core on the FPGA side is encrypted. Therefore, we present an empirical cost model to evaluate the memory throughput $Th_{mem}$. 
In order to predict the memory throughput of MLWeaving, we analyze the memory access pattern of MLWeaving and then benchmark the memory throughput. % according to the memory access pattern 
Note, both ``with chaining" and ``wo chaining" have the same memory subsystem. 

{\bf Memory Access Pattern. }The memory access pattern of MLWeaving is quite fixed. Essentially, for the precision level $s$, it sequentially fetch $s$ cache lines (512 bits) every 32 cache lines, regardless of the number of features. 

{\bf Benchmarking Memory Throughput. }Based on the memory access pattern, we can benchmark the memory throughput for each precision level $s$, as shown in Equation~\ref{E_mem_bandwidth}.  
\begin{equation} \begin{scriptsize}
\label{E_mem_bandwidth}
\vspace{-1ex}
Th_{mem} = \begin{cases}
10.2GB/s &s = 1\\
13.3GB/s &s=2\\
13.8GB/s  & s=3 \\
14.8GB/s  & s\ge  4 \\
\end{cases}
\vspace{-1ex}
\end{scriptsize} \end{equation}

%Direct connection + analytical model. 


==> mlweaving.tex <==
%SGD algorithm relies heavily on the training dataset to compute the gradient which is used to update the model. From the computing's perspective, the training dataset is iteratively scanned before the final model is produced. 
%The training dataset is generally too big to keep inside the processor, i.e., beyond the cache capacity of modern CPU. 

%
%The bit-serial memory layout has the  
%\emph{how to technically gain the linear speedup from using lower precision with only one hardware design?} % and only one index
%\emph{how to technically support any level of precision (with only one hardware design) and gain the linear speedup from using lower precision?} 
%the foundational question we try to answer is \emph{how to use only one hardware design and only one index to efficiently support arbitrary-precision machine learning training?} Accordingly, 


%In this section, we describe what we call the
% \emph{bit-serial design} -- a simplified version of most of the ideas behind
% MLWeaving. Although it cannot be synthesized on
% our FPGA, this can be fixed by further 
% improvements in the final version of MLWeaving. 
 %Similar to MLWeaving,
 %the bit-serial method adopts a hardware/software 
 %co-design approach. In particular, the bit-serial method contains a bit-serial memory layout (software component) and a associated bit-serial arithmetic (hardware component) to achieve the necessary flexibility and high performance, as shown in the ``Bit-serial" column in Table~\ref{t_comparison}. %while maintaining the performance. Besides, the bit-serial method has an appealing property that both memory access and computation time decreases linearly as less bits are used. %answer this question. 

%Deep learning is compute-bound, while linear machine learning is always memory-bound. 


%\texttt{MLWeaving} provides a transposed memory layout, which vertically partitions each sample (containing multiple features) at the bit level. Therefore, \texttt{MLWeaving} can serve its arithmetic units (in hardware side) serial bit stream, i.e., all the first bits of the sample at the first cycle, all the second bits at the second cycle, and so on. It means that the proposed memory layout (having only one index) enables the flexible selection of precision at runtime. And the number of memory transactions (i.e., memory access time) scales linearly with the number of bits used. Therefore, the proposed layout can significantly improve the energy efficiency, since the external memory access is two orders of magnitude more energy-consuming than the arithmetic operation~\cite{inefficiency_gp_isca10, energy_problem_isscc14}. 
%%Specifically, we perform the weaving on the training dataset, based on one observation the  characteristic, benefit
%This is based on the observation that the machine learning algorithm is evaluated in a \emph{sample-at-a-time} manner, i.e., all the features of the sample are scanned before the corresponding gradient is computed. With the proposed memory layout, 



\begin{algorithm} [t!]
	\SetAlFnt{\tiny} \linespread{1.0} \selectfont \caption{\sc Mini-Batch SGD under MLWeaving}
	\label{alg_sgd_flow_bank}
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}	
	
	\begin{scriptsize}
		%	\DontPrintSemicolon
		\Input{$N$: number of samples, \\
			$\gamma$: learning rate, \\
			$Q_s(\vec{a_i})$: $s$-bit quantized data set of the $i$-th sample, $\in \mathbb{F}^{1 \times M}$, \\ %Q_s(\vec{a_i})
			$b_i$: label value of the $n$-th sample, $b_i \in \mathbb{R}^{1}$. }
		
		\Output{$\vec{x}$: model with a set of parameters.}
		
		%\tcc{Add the ($\vec{a_i}, b_i$)'s gradient to $\vec{x}$.}
	\For{($i = 0$; $i < N$; $i += B$)}{
		$\vec{g}$ = 0;	\\
		\For{($j = 0$; $j < B$; $j += \#Bank$)}{

			$\#$pragma parallel in hardware \\
			\For{($k = 0$; $k < \#Bank$; $k++$)}{
				int32 $t = i + j +k$; \\
				\tcc{Dot product of $\vec{Q_s(a_{t})}$ and $\vec{x}$.}
			int32 $a\_dot\_x = Q_s(\vec{a_{t})} \boldsymbol{\cdot} \vec{x}$;
	
			\tcc{$df$ varies with ML algorithm.} %, scalar computation
			int32 $scale = \gamma \times df(a\_dot\_x, b_{i+j+k})$;
			
			\tcc{Compute the gradient for each bank.} % of $i$-th sample
			$\vec{g_{j+k}} = scale \times Q_s(\vec{a_{t}})$;
			
			\tcc{Accumulate the gradient.} % of $i$-th sample
			$\vec{g} = \vec{g} + \vec{g_{j+k}}$;
			}
		}
		\tcc{Accumulate the gradient to $\vec{x}$.} %($\vec{a_i}, b_i$)'s
		$\vec{x} = \vec{x} - \vec{g}$;
	}
	\end{scriptsize}
\end{algorithm}


% \begin{table} [t]
% 	\centering
% 	%\begin{spacing}{0.3}
% 	\begin{scriptsize}
% 		\begin{tabular}{|c||c|c|c|c|c|}
% 			\hline
% 			\textbf{Index} & \textbf{Bank 7:64-bit} & ... & \textbf{Bank 2:64-bit} & \textbf{Bank 1:64-bit} & \textbf{Bank 0:64-bit} \\
% 			\hline
% 			\hline
% 			\hline
% 			$0$ & 7\_63:0\_0 & ... & 2\_63:0\_0 & 1\_63:0\_0 & 0\_63:0\_0  \\
% 			\hline
% 			$1$ & 7\_63:0\_1 & ... & 2\_63:0\_1 & 1\_63:0\_1 & 0\_63:0\_1  \\
% 			\hline
% 			$2$ & 7\_63:0\_2 & ... & 2\_63:0\_2 & 1\_63:0\_2 & 0\_63:0\_2  \\
% 			\hline
% 			$...$ & ... & ... & ... & ... & ...  \\
% 			\hline
% 			$31$ & 7\_63:0\_31 & ... & 2\_63:0\_31 & 1\_63:0\_31 & 0\_63:0\_31  \\
% 			\hline
% 			\hline
% 			$32$ & 7\_127:64\_0 & ... & 2\_127:64\_0 & 1\_127:64\_0 & 0\_127:64\_0  \\
% 			\hline
% 			$33$ & 7\_127:64\_1 & ... & 2\_127:64\_1 & 1\_127:64\_1 & 0\_127:64\_1  \\
% 			\hline
% 			$...$ & ... & ... & ... & ... & ...  \\
% 			\hline
% 			\hline
% 			$1024$ & 15\_63:0\_0 & ... & 10\_63:0\_0 & 9\_63:0\_0 & 8\_63:0\_0  \\
% 			\hline
% 			$1025$ & 15\_63:0\_1 & ... & 10\_63:0\_1 & 9\_63:0\_1 & 8\_63:0\_1  \\
% 			\hline
% 			$...$ & ... & ... & ... & ... & ...  \\
% 			\hline
% 		\end{tabular}
% 		\label{t_mlweaving_instance}
% 		\vspace{-1ex}	
% 		\caption{Instantiation of MLWeaving memory layout. \emph{x\_y:z\_w} denotes the \emph{w}-th bits of 64 features (from $z$-th to $y$-th) in the $x$-th sample and $y - z = 63$. A row contains a cache line (512 bits). }
% 		\vspace{-2ex}
% 	\end{scriptsize}
% 	%\end{spacing}
% \end{table}


\section{MLWeaving} %: Flexibility \& Performance \& Deployment
\label{sec_ml_weaving}

MLWeaving develops the ideas behind BSM so as to make them implementable. In particular, MLWeaving changes both the memory layout and the design on the FPGA to reduce the required bitwidth of the model.

Inspired by mini-batch SGD which uses the same model to process one mini batch of $B$ samples\footnote{In our current design, $B$ should be a multiple of 8.}, MLWeaving adopts a multi-bank hardware design for the ML training (Algorithm~\ref{alg_sgd_flow_bank}). 
In particular, 8 physical banks are instantiated to accommodate 8 samples simultaneously (Line 4) that are processed in a lock-step manner. Since $B$ samples in the same mini batch read the same model (Line 7), MLWeaving takes advantage of this property to reduce the model bitwidth without compromising on any throughput. In the following, we present the memory layout and hardware design of MLWeaving.%Next, we show the intuition behind MLWeaving, followed by the related memory layout and hardware design.
%With this approach, MLWeaving is more amenable to hardware implementation, while maintaining precision flexibility and high throughput (i.e., $\#CL$ bits per cycle), as shown in Table~\ref{t_comparison}.

%In the BSM design in Figure~\ref{fig_bit_serial_hardware}, a cache line contains the x-bit of 512 features for a given sample. In MLWeaving, a cache line contains the x-bit of 256 features of sample $n$ and 256 features of sample $n$+1 (for the case with 2 banks). So while bit-serial processes, in principle, data form a single sample (row) in a cycle, MLWeaving processes data from 64 rows (samples) per cycle but less bits for each one of them. Thus, each cycle in MLWeaving processes less data from a sample (using a bank) but it processes several samples, while bit-serial processes one sample at a time. Since all the samples processed in all the banks correspond to the same part of the model, MLWeaving only needs to read that part of the model for all banks. Therefore, the bitwidth becomes 2K bits under MLWeaving, compared with 16K bits under bit-serial. 



\begin{figure*}
	\centering
	\subfloat[Overall architecture]{\includegraphics[width=3in]{mlweaving_hw_overall.pdf} 
		\label{fig_mlweaving_overall}} % \caption{}
	%\hfill
	\subfloat[Detailed design of each bank]{\includegraphics[width=2.4in]{mlweaving_hw_bank.pdf} \label{fig_mlweaving_bank}} % \caption{}
	\caption{Arithmetic of MLWeaving. For the instantiation, $\#CL$ is 512 and $\#Bank$ is 8. } 
	\vspace{-1.5ex}
	\label{fig_mlweaving_hw} 
	\vspace{-2ex}
\end{figure*}  


	\vspace{-1ex}
\subsection{MLWeaving Memory Layout (Software)} 
\label{subsec_mlweaving_layout}
	\vspace{-0.5ex}
% partitioning each sample at the bit level, 
%The objective of MLWeaving memory layout can provide the exact bit-serial stream to the corresponding hardware design, such that the performance and energy efficiency is guaranteed.  
%No resource overhead is due to the fact that the data flows into the computing pipeline smoothly, without any 
%The bit-serial memory layout saturates the entire $CL$-bit memory transaction with the bits from a single sample (i.e., only exploring intra-sample parallelism). In contrast, each memory transaction assembles the data from $\#Bank$ samples, each of which contributes $\frac{\#CL}{\#Bank}$ bits under MLWeaving. 
Starting from the BSM memory layout in Figure~\ref{fig_bit_serial_layout}, we show the memory layout transition to MLWeaving in Figure~\ref{fig_mlweaving_bank_layout}. 
BSM saturates each memory transaction with eight bits from the same row, e.g., {\color{blue} AEIMRV10} of the first row. In contrast, the first/second row contributes four bits for each memory transaction under MLWeaving. For instance, the first bits of the first four features of two rows assemble into the first memory transaction, e.g., {\color{blue} AEIMaeim}. %It can perf
Since the bits {\color{blue} AEIM} and {\color{blue} aeim} share the same weights, the model only needs to provide four weights within a cycle. %contains four bits from the first row and four bits from the second row 


{\bf Instantiation of Memory Layout.} We instantiate the MLWeaving memory layout by setting $\#CL$ (or $\#Bank$) to be 512 (or 8). Now we use the case with $M$ = 2048 as an example in Table~\ref{t_bit_serial_instance}. For instance, the first memory transaction is populated with the first bits of the first 64 features of the first eight samples. If $M$ is not a multiple of 64, we use padding to align it to 64 bits. \wzk{So the memory traffic $MT$ (in terms of bits) for each sample contains two sources, as shown in Equation~\ref{E_memory_traffic}. The first part indicates the memory traffic from all the features, evaluated to be the precision level $s$ multiplied by the value which rounds up $M$ to the nearest multiple of 64. The second part (32 bits) comes form the label of each sample. }
\begin{equation} \begin{scriptsize}
\label{E_memory_traffic}
	\vspace{-1ex}
MT = s \times \lceil \frac{M}{64} \rceil \times 64 + 32
	\vspace{-1ex}
\end{scriptsize} \end{equation}

%Suppose we want to achieve 8-way parallelism ($\#CL$ = 8).   
 
%MLWeaving also exploit not only intra-sample $\frac{CL}{\#Bank}$-way parallelism, but also inter-sample $\#Bank$-way parallelism. 
%In particular, we 
%to share the memroy transaction with multiple samples. 

%Each $\#CL$-bit memory transaction contains features from $\#Bank$ rows. 
%Serial part: 

\begin{table} [t]
	\centering
	%\begin{spacing}{0.3}
	\begin{scriptsize}
		\begin{tabular}{|p{1.6cm}|c||c|c|c|c|}
			\hline
			\textbf{Description} &\textbf{Index} & \textbf{Bank 7} & ... & \textbf{Bank 1} & \textbf{Bank 0} \\
			\hline
			\hline
			\hline
			\multirow{6}={First 64 features of the first 8 samples}&$0$ & 7\_63:0\_0 & ... & 1\_63:0\_0 & 0\_63:0\_0  \\
			\cline{2-6}
			&$1$ & 7\_63:0\_1 & ... &  1\_63:0\_1 & 0\_63:0\_1  \\
			\cline{2-6}
			&$2$ & 7\_63:0\_2 & ... &  1\_63:0\_2 & 0\_63:0\_2  \\
			\cline{2-6}
			&$...$ & ... & ... & ... & ...  \\
			\cline{2-6}
			&$31$ & 7\_63:0\_31 & ... & 1\_63:0\_31 & 0\_63:0\_31  \\
			\hline
			\hline
			\multirow{3}={Second 64 features of the first 8 samples} & $32$ & 7\_127:64\_0 & ... & 1\_127:64\_0 & 0\_127:64\_0  \\
			\cline{2-6}
			&$33$ & 7\_127:64\_1 & ...  & 1\_127:64\_1 & 0\_127:64\_1  \\
			\cline{2-6}
			& $...$ & ... & ... & ...  & ...  \\
			\hline
			\hline
			$...$ & $...$ & ... & ... & ...  & ...  \\
			\hline
			\hline
			\multirow{3}={First 64 features of the second 8 samples}&$1024$ & 15\_63:0\_0 & ... & 9\_63:0\_0 & 8\_63:0\_0  \\
			\cline{2-6}
			&$1025$ & 15\_63:0\_1 & ... & 9\_63:0\_1 & 8\_63:0\_1  \\
			\cline{2-6}
			&$...$ & ... & ... & ... & ...  \\
			\hline
		\end{tabular}
		\label{t_mlweaving_instance}
		\vspace{-1ex}	
		\caption{Instantiation of MLWeaving memory layout. \emph{x\_y:z\_w} denotes the \emph{w}-th bits of 64 features (from $z$-th to $y$-th) in the $x$-th sample and $y - z = 63$. A row contains a cache line (512 bits). }
		\vspace{-2ex}
	\end{scriptsize}
	%\end{spacing}
\end{table}


\vspace{-1ex}
\subsection{MLWeaving Arithmetic (Hardware)} %
\label{subsec_mlweaving_arithmetic}
Following Algorithm~\ref{alg_sgd_flow_bank}, we present the detailed hardware design of MLWeaving in Figure~\ref{fig_mlweaving_hw}. 
%The targeted processing rate (high performance) is $\#CL/s$, where $s$ is the %precision level at runtime.
In the following, we explain the overall architecture, followed by the details inside a bank. 

\begin{figure}[t]
	\centering
	\includegraphics[width=6cm]{bit_serial_to_mlweaving.pdf}
	\vspace{-1.5ex}
	\caption{BSM memory layout (a) converted to MLWeaving memory layout (b). An example of $\#CL$ (8), $\#Bank$ (2) and $M$ (8). } %The model only needs to provide four weights per cycle under MLWeaving, compared with eight under bit-serial.
	\vspace{-1ex}
	\label{fig_mlweaving_bank_layout}
\end{figure}

\begin{table} %[!hbp]
	\centering
	%\begin{spacing}{0.3}
	\begin{scriptsize}
	\begin{tabular}{|c||c|c|c|c|}
		\hline
		\textbf{Name} & \textbf{Logic (ALMs)} & \textbf{DSPs} & \textbf{BRAMs} & \textbf{Frequency} \\ 
		\hline
		\hline
		\textbf{BSM} & N.A & N.A & N.A & N.A\\
		\hline	
		\textbf{MLWeaving} & 35670 (8.4\%) & 0 (0\%) & 3.25Mb  (6.1\%) & 400 MHz\\
		\hline
	\end{tabular}
		\vspace{-1ex}
 	\caption{Resource consumption }
	\label{t_resource_conparison}
	\vspace{-4ex}
	\end{scriptsize}
	%\end{spacing}
\end{table}


In the ``multi-bank" processing stage, the 512-bit computing pipeline is divided into 8 banks, each of which consumes 64 bits from one sample (\circled{1}), as shown in Figure~\ref{fig_mlweaving_overall}. %Now, the model ($\vec{x}$) only needs to provide $32 * \#CL/\#Bank$ bits per cycle and broadcast them to all the banks. 
In the ``gradient accumulation" stage, the gradient (width: 2K) of each bank is fed to 64 element-wise adder trees which generate the accumulated gradient (\circled{2}). %In other words, $\#Bank$-way inter-sample parallelism is exploited. 
%We can see that the adder trees and model are fully pipelined.  (e.g., s)
In the ``model update" stage, the accumulated gradient is used to update the working model ($\overrightarrow{x\_w}$) (\circled{3}) for every 8 samples. Meanwhile, the architectural model ($\vec x$) is updated only after a mini batch ($B$) of samples. %It mean that the width of the model 
% Each bank provides $\#CL/\#Bank$-way intra-sample parallelism. 
Inside a bank, it behaves the same as that in the BSM arithmetic in Figure~\ref{fig_bit_serial_hardware}, except that each bank instantiates 64 bit-serial multipliers in the ``dot product" and ``gradient computation" stages. Since we instantiate 8 banks, the total throughput of the MLWeaving arithmetic is still 512 bits per cycle. 


{\bf Instantiation of hardware design. }
Figure~\ref{fig_mlweaving_hw} illustrates the instantiation of MLWeaving with $\#CL = 512$ and $\#Bank = 8$. Table~\ref{t_resource_conparison} shows the resource consumption in our FPGA when implementing the computing pipeline in MLWeaving. MLWeaving achieves high frequency (400MHz) while requiring a reasonable amount of FPGA resources. This is because 1) the proposed multi-bank architecture of MLWeaving leads to less BRAMs (on-chip memory on FPGAs) for the architectural and working models in Figure~\ref{fig_mlweaving_hw}, and 2) MLWeaving memory layout allows the MLWeaving hardware design to directly consume the data from memory, without auxiliary hardware modules for transposition. The throughput of MLWeaving hardware design can roughly reach 25.6GB/s (400M * 512 bits per cycle), much larger than the existing memory bandwidth: 15GB/s. 

 

%the system computes the gradient for the correspond sample (Figure~\ref{fig_mlweaving_bank}). Its output gradient, whose width is $32 * \#CL/\#Bank$ bits, is fed into the gradient accumulation module (Line 8). The hardware details inside the bank are described as follows.
%First, the bank accepts $\#CL/\#Bank$ bits, each of which is served by a bit-serial multiplier. In other words, $\#CL/\#Bank$-way intra-sample parallelism is exploited. 
%Second, the dot product is computed (Line 5). Since each bit-serial multiplier needs $s$ cycles to compute one multiplication, the processing rate of the dot product part is $\#CL/(s *\#Bank)$ features per cycle. 
%Third, the scaling value is calculated (Line 6). Its computation is fully pipelined. 
%Fourth, the gradient computation (Line 7) is performed using $\#CL/\#Bank$ bit-serial multipliers. Therefore, its processing rate is also $\#CL/(s *\#Bank)$ features per cycle.  

%It also takes $s * \lceil \cfrac{M}{\#CL/\#Bank} \rceil$ cycles to produce the gradient. Again, the gradient computation times grows linearly with $s$.
%It takes $s * \lceil \cfrac{M}{\#CL/\#Bank} \rceil$ cycles to produce one dot product of the sample, where $s$ is the precision level used during the training, $\lceil \cfrac{M}{\#CL/\#Bank} \rceil$ is fixed number of chunks for a sample. Therefore, the computation time of the dot product grows linearly with the number ($s$) of bits used. 

%In summary, the processing rate of each bank, e.g., $\#CL/(s *\#Bank)$ features per cycle, is determined by the slowest parts (dot product and gradient computation). %our objective is accomplished. \emph{MLWeaving can provide both flexibility and high performance}.   

%$32 * \#CL/\#Bank$

%The overall architecutre
%Instead The overall architecture contains $\#Bank$ banks, which share the model $\vec{x}$, so the bitwidth of $\vec{x}$ becomes $32*\#CL/\#Bank$.

%parallel part: both dot-product and gradient computing is embarrassingly parallel.  



%The overall architecture contains $\#Bank$ banks, which share the model $\vec{x}$, so the bitwidth of $\vec{x}$ becomes $32*\#CL/\#Bank$.



==> system_overview.tex <==
%\vspace{-1ex}
\section{System Overview} %: Pitfalls of Existing Low-precision Designs

\vspace{-1ex}
\subsection{\kaan{Database Integration}}
\kaancomment{Should we introduce Xeon+FPGA also around here with a figure?}

We integrate our FPGA-accelerated training designs into DoppioDB~\cite{sidler2017doppiodb}, an open source solution for FPGA-accelerated databases, based on MonetDB~\cite{idreos2012monetdb}. DoppioDB enables easy integration of FPGA-based accelerators through a set of software and hardware libraries~\cite{centaur_fccm17}. The hardware libraries expose a native memory interface which the FPGA accelerators use to access the main memory of the host CPU. On the software side, FPGA accelerators can be started and monitored as separate threads. These FPGA threads run in parallel to software threads.

We implement three User Defined Functions (UDF) in DoppioDB: (1) The first UDF is to initiate the creation of the MLWeaving data structure. This data structure is kept internal in the database, similar to an index, associated with a certain table. (2) The second UDF is to initiate training using MLWeaving. Under the hood, DoppioDB will look for the MLWeaving index that belongs to the table given by this UDF. If found, the FPGA thread is started. It uses MLWeaving index to train a model which then gets transferred to the main memory. (3) The third UDF is to perform inference on tuples using the model that has been trained before. Similar to the MLWeaving index, the trained model is also associated with a certain table and will check during query execution if inference can be performed, conditioned on a model having been trained before.

With MlWeaving integrated into DoppioDB, users have a SQL front-end for training models over relational data in a seamless manner as the preparation and selection of data needed before training can be done using SQL. 

\vspace{-1ex}
\subsection{Design Methodology}
Since MLWeaving involves many aspects that interact in a tight manner, we present the ideas behind MLWeaving in three stages: ``Quantized''~\cite{sgd_fpga_fccm17}, ``MLWeaving\_NP" (Section~\ref{sec_bit_serial_method}) and ``MLWeaving" (Section~\ref{sec_ml_weaving}), as illustrated in Table~\ref{t_comparison}. 
For a better understanding of MLWeaving, it is important to understand the interplay between the data representation and the processing required by the accelerator. In the case of SGD, the most important components in the design is the computing circuits and how data is transferred from the external memory (the input data) and accessing the model on FPGA local memory. 


{\bf Computing Circuits. }``Quantized'' employs fixed circuits for each precision level, so it requires the data to be available at the corresponding precision and processes features using fixed-point bit-parallel multipliers. However, ``MLWeaving\_NP" and ``MLWeaving" use bit-serial multipliers~\cite{bit_serial_assp89}, which enable on-the-fly precision selection. We conclude that ``Quantized'' can support one precision level while both ``MLWeaving\_NP" and ``MLWeaving" can support 32 levels.   %``MLWeaving\_NP" uses a serial design for multipliers. This design does not scale for SGD so the final design in ``MLWeaving" is also bit-serial but includes a data partitioning feature to make it \kaan{\st{workable} more efficient} in an FPGA (both designs will be described \kaan{in Section X\st{later on in the paper}}). The comparison between these approaches is included to help understand how the memory layout affects the FPGA design for those less familiar with FPGA programming. \kaan{\st{and will be used later on in the paper.}}

%First we describe the bit-serial method (Section~\ref{sec_bit_serial_method}) that achieves high performance but cannot be directly implemented. Then we describe MLWeaving (Section~\ref{sec_ml_weaving}).
%\kaancomment{Is it a good idea to refer to figures that come much later in the paper? I would modify this paragraph.}
%The description of the data structure used to store the data is also organized in stages: it evolves from the basic quantized table shown in Figure~\ref{fig_quantization} to the bit-serial format in Figure~\ref{fig_bit_serial_layout} and finally to the MLWeaving solution shown in Figure~\ref{fig_mlweaving_bank_layout}. For the hardware design, the SGD arithmetic is evolved from the original quantized design to the bit-serial arithmetic in Figure~\ref{fig_bit_serial_hardware} and then to the approach adopted in MLWeaving in Figure~\ref{fig_mlweaving_hw}. % in Figure~\ref{fig_quantizated_hardware}  

% shows a comparison between three possible designs for low precision SGD on an FPGA. 
 


{\bf Memory Layouts. }In the Xeon+FPGA platform~\cite{centaur_fccm17} used to implement MLWeaving, the FPGA \st{is cache coherent with the CPU}\kaan{ has cache coherent access to the main memory of the CPU}. The data arrives to the FPGA from the memory of the CPU in the form of cache lines, {\em \#CL} (512 bits per cache line in our platform). Efficiency is achieved by processing as many elements within that cache line as possible. How many elements are within a cache line depends on how the data is stored in memory. Hence it is important to have an appropriate representation for the data. ``Quantized'' stores the data for a given precision in a consecutive manner.
If the precision is 16 bits, every cache line brings in 512/16 dimensions (e.g., features or columns) to be processed. Because the value for each dimension arrives as a whole, the multipliers needed for the gradient computation are based on the 16-bits used to represent a value. Such 16-bit wide multipliers are complex and take up significant space. 
In ``MLWeaving\_NP" and ``MLWeaving", the data is represented in memory not as a sequence of values but as a sequence of bits of different values. For instance, reading a cache line brings in the first bit of 512 dimensions.
Thus, we cannot compute the gradient for a value right away. Instead, we use a bit-serial multiplier, where the required multiplication is performed one bit at a time with the result accumulated and added to the next one-bit multiplication until the whole multiplication is completed on a value. As such, ``MLWeaving\_NP" and ``MLWeaving" use one memory layout to support arbitrary-precision data retrieving from memory, while ``Quantized'' requires one memory layout for each precision level. %As we will show later, this can be very efficiently implemented in an FPGA, both in terms of resources and speed.
%\kaancomment{Again, this paragraph dives in to details too early. It is not clear why we give this information here. Should we create a subsection here as well and say we are comparing non-bitserial with bitserial?}[3cm]

{\bf Accessing the Model on FPGAs. }The dot product in SGD involves not only the input data but also the corresponding entry in the model. Thus, an additional factor of complexity in the design is reading the corresponding values of the model. A design that operates over complete values for each dimension needs to read the values from the model also as a whole. This is referred to the {\em bitwidth of the model}. The bitwidth is a very important parameter in an FPGA design because it affects the complexity of the interconnects and the way data has to move from the model storage to the computing units. The higher the bit-width, the more complex the design and, thus, the higher probability that it will not meet timing at higher clock rates. 
``Quantized'' processing dimensions as a whole has a model bitwidth of $\lfloor\tfrac{512}{s}\rfloor \times 32$, where the precision of the model is 32 bits and $s$ is the precision level of input data. 
``MLWeaving\_NP" has a high model bitwidth of $16K$ (32*512)\footnote{In Intel Arria 10 FPGA~\cite{Intel_arria_10_device}, the model is implemented with 20-Kb memory blocks (i.e., M20Ks). Each M20K can provide a 32-bit width with ECC (or 40-bit without ECC) for the model, so a 16K-bit width requires 512 M20Ks with ECC (or 410 without ECC). It is extremely difficult to access 410 M20Ks in a lock-step manner while maintaining high frequency, as M20Ks are distributed in an FPGA. }, making it unsuitable in real settings. 
``MLWeaving" reduces the bitwidth of model by using mini-batch SGD algorithm (Subsection~\ref{subsection_lp_sgd}) where one mini batch is processed without modifying the model. This allows MLWeaving to adopt a multiple-bank hardware design (similar to data partitioning but in hardware) such that each bank can accommodate a sample. The hardware design of MLWeaving has 8 banks, each bank only needs to consume 64 bits to achieve the necessary throughput, 512 bits per cycle. Since all the banks share the same model, the model bitwidth becomes 2K, significantly smaller than 16K of ``MLWeaving\_NP" which literally uses only one bank. About the supported mini-batch size $B$, ``MLWeaving" can only support the size $B$, which is a multiple of 8, while the other two can support any positive integer size.

\begin{table} %[!hbp]
	\centering
	%\begin{spacing}{0.3}
	\begin{scriptsize}
		\begin{tabular}{|c||c|c|c|}
			\hline
			\textbf{Hardware Metrics}& \textbf{Quantized}~\cite{sgd_fpga_fccm17} & \textbf{BSM} & \textbf{MLWeaving} \\
			\hline
			\hline
			Supported precision levels & $s$-bit only  &  1-32 & 1-32 \\
			\hline
			Required memory layouts &  One for $s$-bit  &  Shared & Shared \\
			\hline
			%Degree of intra-sample parallelism & $\lfloor \tfrac{\#CL}{s} \rfloor$ &  $\#CL$ & $\tfrac{\#CL}{\#Bank}$ \\
			%\hline
			%Degree of inter-sample parallelism & 1 &  1 & $\#Bank$ \\
			%\hline
			%Model update pattern & Async & Sync & Sync \\
			%\hline
			Bitwidth (bits) of model $\vec{x}$ &   $\lfloor\tfrac{512}{s}\rfloor \times 32$  &  16K & 2K  \\
			\hline
			Number of banks, $\#Bank$ &  1  &  1 & 8 \\
			\hline			
			Mini-batch size, $B$ &  n  &  n & 8*n \\
			\hline			
			%\hline
			%\hline
			%\emph{Performance metrics} &  &  &  \\
			%\hline
			%Throughput (bits/cycle) & $s \times \lfloor \tfrac{\#CL}{s} \rfloor$   &  $\#CL$ & $\#CL$ \\
			%\hline
			%Processing rate (features/cycle) & $\lfloor \tfrac{\#CL}{s} \rfloor$   &  $\tfrac{\#CL}{s}$ & $\tfrac{\#CL}{s}$ \\			
			%\hline
			%Frequency & Moderate  &  Low & High \\
			%\hline
			%$\lfloor 512/s \rfloor \times 32$
		\end{tabular}
	\vspace{-2ex}
	\caption{Comparison of three approaches. $\#CL$ is 512 and $\#Bank$ is 8.}
		\label{t_comparison}
		\vspace{-3ex}
	\end{scriptsize}
	%\end{spacing}
\end{table}
%, $s$ is the precision level.


%SGD has attracted intensive
%interests recently. We summarize the property and
%limitations of a recent hardware design~\cite{sgd_fpga_fccm17},
%and present a high-level comparison with two 
%strategies that we propose in this work.

%We take the low-precision SGD in $s$-bit precision~\cite{sgd_fpga_fccm17} as an example (the ``Quantized" column in Table~\ref{t_comparison}). This implementation 
%uses small-area multiplier (e.g., $s \times 32$) and a tightly padded $s$-bit quantized data representation are employed to maximize performance and energy efficiency. 

%{\bf Supported precision levels. } Only one precision level (i.e., $s$) is supported by the $s$-bit SGD arithmetic. 

%{\bf Required storage layouts. } One quantized storage layout is needed by the $s$-bit SGD arithmetic. 

%{\bf Degree of intra-sample parallelism.} The \emph{intra-sample parallelism} indicates that the hardware design explores the parallelism among features inside a sample. ``Quantized" achieves $\lfloor \#CL/s \rfloor$-way intra-sample parallelism. This means that the lower the precision (e.g., $s$-bit), the higher the degree of intra-sample parallelism. 

%{\bf Degree of inter-sample parallelism.}
%The \emph{inter-sample parallelism} indicates that the hardware design explores the parallelism among samples. Specifically, different samples enter the computing pipeline simultaneously. Under ``Quantized", the degree of inter-sample parallelism is 1, since the second sample enters the computing pipeline after the first sample. %has already been processed. %Therefore, it is 1. 

%{\bf Bitwidth of the model ($\vec{x}$).}
%The bitwidth of the model, which resides in on-chip memory, mainly determines the implementation complexity of SGD hardware design. 
%Typically, the larger bitwidth, the more complexity. 
%``Quantized" exploits $\lfloor \#CL/s \rfloor$-way intra-sample parallelism, so $\lfloor \#CL/s \rfloor$ features in the same sample can enter the computing pipeline within a cycle. Accordingly, the model ($\vec{x}$) needs to provide $\lfloor \#CL/s \rfloor$ weights within a cycle, since each feature in the sample requires one distinct weight for the corresponding dot product. 
%Suppose each weight has 32 bits, the total bitwidth of the model becomes $\lfloor \#CL/s \rfloor \times 32$ bits. %When $s$ is 1 or 2, the pipeline width ($\#CL$) is halved due to the fact that the bitwidth of the model is too large~\cite{sgd_fpga_fccm17}.  
% Since 
 
%{\bf Model update pattern.} 
%The model update pattern of SGD can be synchronous or asynchronous. Synchronous SGD indicates that the semantics of SGD in Algorithm~\ref{alg_sgd_flow} is preserved, while asynchronous SGD is violated. ``Quantized" adopts asynchronous SGD for better computation speed. 

%\subsubsection{Performance Metrics}
%Two metrics are used to evaluate the performance of $s$-bit-precision machine learning. % in $s$-bit precision. 

%{\bf Throughput (bits/cycle).}
%``Quantized" can consume $\#CL$ bits from external memory within a cycle. Therefore, its throughput is $\#CL$ bits per cycle. %and $\#CL$ is the pipeline width (e.g., 512 bits). 

%{\bf Processing rate (features/cycle).} 
%The $\#CL$-bit computing pipeline of ``Quantized" can accept $\lfloor \#CL/s \rfloor$ features within a cycle. So its processing rate is $\lfloor \#CL/s \rfloor$ features per cycle. 
%Each sample with $M$ features can be processed in $\lceil \cfrac{M}{\lfloor \#CL/s \rfloor} \rceil$ cycles. 


%{\bf  }
%After the analysis of the existing design, we identify our objective and solution presented in this paper. 

%{\bf Objective. }
%Our objective is four-fold. First, any level of precision is supported with only one hardware design and one storage layout (flexibility). Second, its processing rate, i.e., $\tfrac{\#CL}{s}$, is comparable to the $s$-bit quantized design (performance). Third, it is amenable to real hardware implementation (ease of deployment). Fourth, it is synchronous. 

%{\bf Our solution. }

